An efficient Lagrangian-based heuristic to solve a multi-objective sustainable supply chain problem

Sustainable Supply Chain (SSC) management aims at integrating economic, environmental and social goals to assist in the long-term planning of a company and its supply chains. There is no consensus in the literature as to whether social and environmental responsibilities are profit-compatible. However, the conflicting nature of these goals is explicit when considering specific assessment measures and, in this scenario, multi-objective optimization is a way to represent problems that simultaneously optimize the goals. This paper proposes a Lagrangian matheuristic method, called $AugMathLagr$, to solve a hard and relevant multi-objective problem found in the literature. $AugMathLagr$ was extensively tested using artificial instances defined by a generator presented in this paper. The results show a competitive performance of $AugMathLagr$ when compared with an exact multi-objective method limited by time and a matheuristic recently proposed in the literature and adapted here to address the studied problem. In addition, computational results on a case study are presented and analyzed, and demonstrate the outstanding performance of $AugMathLagr$.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

==> tables/table_sets_flow.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[htb]
\begin{center}
\scriptsize
\tabcolsep=0.5cm
\caption{Description of the in- and out-flow of items in entities in the studied SC.}
\label{tab:sets_flow}
\begin{tabular}{lll}
%\rowcolor[HTML]{FFF} 
\hline
\textbf{Definition}& \textbf{Set}     & \textbf{Description}      \\ \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{tabular}[c]{@{}l@{}}In-flow of \\ final products ($fp$)\\ in factories\end{tabular}     
& $F_{INFFP}$                                                                            
& \begin{tabular}[c]{@{}l@{}}Factories can receive $fp {\in M_{fp}}$ from:\\ -- other factories;\\ -- warehouses (in case of assembled goods, for example);\\ -- airports and airports through cross-docking.\end{tabular}                                                                                           \\ \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{tabular}[c]{@{}l@{}}Out-flow of\\ final products ($fp {\in M_{fp}}$)\\ in factories\end{tabular}     
& $F_{OUTFFP}$                                                                   
& \begin{tabular}[c]{@{}l@{}}Factories can send $fp$ to:\\ -- factories;\\ -- warehouses;\\ -- directly to customers;\\ -- seaports and airports through cross-docking.\end{tabular}                                                                                                                    \\ \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{tabular}[c]{@{}l@{}}In-flow of recovered\\products ($rp$)\\in factories\end{tabular} 
& $F_{INFRP}$                                                                       
& \begin{tabular}[c]{@{}l@{}}Factories can receive $rp$ from:\\ -- warehouses;\\ -- directly from customers;\\ -- seaports or airports through cross-docking.\end{tabular}                                                                                                                              \\ \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{tabular}[c]{@{}l@{}}In-flow in\\warehouses\end{tabular}                                                                        
& \textbf{$F_{INW}$}                                                    
& \begin{tabular}[c]{@{}l@{}}- Warehouses can receive:\\ -- $fp$ from factories or other warehouses;\\ -- $rp$ from customers or other warehouses;\\ -- $fp$ or $rp$ to airports or seaports through cross-docking.\\
\end{tabular}     \\ \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{tabular}[c]{@{}l@{}}Out-flow in\\warehouses\end{tabular}                                                                       
& $F_{OUTW}$                    & \begin{tabular}[c]{@{}l@{}}- Warehouses can send:\\ -- $fp$ to factories, other warehouses or customers;\\ -- $rp$ to factories or other warehouses;\\ -- $fp$ or $rp$ to airports or seaports through cross-docking.\\
\end{tabular} \\ \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{tabular}[c]{@{}l@{}}In-flow in airports\\ and seaports\end{tabular}
& \begin{tabular}[c]{@{}l@{}}$F_{INAIR}$,\\ $F_{INPORT}$\end{tabular}
& \begin{tabular}[c]{@{}l@{}}Airports and seaports can receive:\\ -- rm from suppliers;\\ -- fp from factories or warehouses;\\ -- rp from warehouses or customers;\\ -- rm, fp or rp from other airports or seaports through cross-docking.\end{tabular}                                     \\ \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{tabular}[c]{@{}l@{}}Out-flow in airports\\ and seaports\end{tabular}     
& \begin{tabular}[c]{@{}l@{}}$F_{OUTAIR}$,\\ $F_{OUTPORT}$\end{tabular} 
& \begin{tabular}[c]{@{}l@{}}Airports and seaports can send:\\ -- $rm$ to factories;\\ -- $fp$ to factories, warehouses or customers;\\ -- $rp$ to factories or warehouses;\\ -- $rm, fp$ or $rp$ to other airports or seaports through cross-docking.\end{tabular}                                             \\ \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{tabular}[c]{@{}l@{}}In-flow of\\ final products ($fp$)\\ in customers\end{tabular}      
& $F_{INCFP}$                                                          & \begin{tabular}[c]{@{}l@{}}Customers can receive $fp$ from:\\ --factories or warehouses.\end{tabular}                                                                                                                                                                                                  \\ \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{tabular}[c]{@{}l@{}}Out-flow of recovered\\products ($rp$)\\ in customers\end{tabular} & $F_{OUTCRP}$                                                          
& \begin{tabular}[c]{@{}l@{}}Customers can send $rp$ to:\\ -- factories;\\ -- warehouses (warehouses can act as sorting centers);\\ --  airports and airports through cross-docking.\end{tabular}                      \\ \hline 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{tabular}
\end{center}
\end{table}
